Dynamic Resource Allocation in Distributed MIMO-LEO Satellite Networks

This paper characterizes the impacts of channel estimation errors and Rician factors on achievable data rate and investigates the user scheduling strategy, combining scheme, power control, and dynamic bandwidth allocation to maximize the sum data rate in the distributed multiple-input-multiple-output (MIMO)-enabled low earth orbit (LEO) satellite networks. However, due to the resource-assignment problem, it is challenging to find the optimal solution for maximizing the sum data rate. To transform this problem into a more tractable form, we first quantify the channel estimation errors based on the minimum mean square error (MMSE) estimator and rigorously derive a closed-form lower bound of the achievable data rate, offering an explicit formulation for resource allocation. Then, to solve the NP-hard problem, we decompose it into three sub-problems, namely, user scheduling strategy, joint combination and power control, and dynamic bandwidth allocation, by using alternative optimization (AO). Specifically, the user scheduling is formulated as a graph coloring problem by iteratively updating an undirected graph based on user requirements, which is then solved using the DSatur algorithm. For the combining weights and power control, the successive convex approximation (SCA) and geometrical programming (GP) are adopted to obtain the sub-optimal solution with lower complexity. Finally, the optimal bandwidth allocation can be achieved by solving the concave problem. Numerical results validate the analytical tightness of the derived bound, especially for large Rician factors, and demonstrate significant performance gains over other benchmarks.

==> proof.tex <==
\begin{appendices}
\section{Proof of Theorem \ref{MRC_SINR_T}}
\label{Prooftheorem1}

From (\ref{kth_SINR}), we need to derive the expressions of ${\left| {{\rm{DS}}_{k}} \right|^2}$, $\mathbb{E}\left( \left| {{\rm{LS}}_{k}} \right|^2 \right)$, $\mathbb{E}\left( \left| {{\rm{UI}}_{k,k'}} \right|^2 \right)$ and $\mathbb{E}\left( \left| {{\rm{N}}_{k}} \right|^2 \right)$, respectively.

We first rewrite the expression of the estimated channel \(\mathbf{\hat h}_{m,k}\) as
\begin{equation}
    \label{rwestimatedchennel}
    \begin{split}
    \mathbf{\hat h}_{m,k} &= \sqrt{\frac{{\bar K}_{m,k}}{{\bar K}_{m,k}+1}}\sqrt{\beta_{m,k}}\mathbf{\bar{h} }_{m,k} + \sqrt{\tau p_k^p}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k} \Big(\sum_{j \in \mathcal{P}_k}\sqrt{\frac{\tau p^p_j\beta_{m,j}  }{{\bar K}_{m,j}+1}}\mathbf{\widetilde h}_{m,j} +{\bf{n}}_{m,k}^p \Big) \\
    & = {{\sqrt{\bar K_{m,k}a_{m,k}}\mathbf{\bar{h} }_{m,k}}}  + \underbrace{\sqrt{\tau p_k^p}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\Big(\sum_{j \in \mathcal{P}_k}\sqrt{\tau p^p_j a_{m,j}}\boldsymbol{\Delta}_{m,j}^{\frac{1}{2}}\mathbf{\widetilde h}_{m,j} +{\bf{n}}_{m,k}^p \Big)}_{\mathbf{\widetilde q}_{m,k}}.
    \end{split}
\end{equation}
The channel \(\mathbf{ h}_{m,k}\) can be rewritten as
\begin{equation}
    \mathbf{ h}_{m,k} = \sqrt{\bar K_{m,k}a_{m,k}}\mathbf{\bar{h} }_{m,k} + \sqrt{a_{m,k}}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}} \mathbf{\widetilde h}_{m,k}.
\end{equation}

Then, we compute ${\rm{DS}}_k$. Since estimated channel $\hat {\bf{h}}_{m,k}$ and estimation error $\mathbf{h}_{m,k}-\hat {\bf{h}}_{m,k}$ are independent, we have
\begin{equation}
\label{MRC_DSk}
\begin{split}
	{{\rm{DS}}_{k}}  &= { \mathbb{E}{\left\{ {\sum\limits_{m \in {\mathcal{M}}_k} { {{w_{m,k}p_k^d}} {{ {{\bf{\hat h}}^H_{m,k}} }} {{\bf{\hat h}}_{m,k}}} } \right\}} }  \\
	 &= {\sqrt{p_k^d}}  \sum\limits_{m \in {\mathcal{M}}_k} {w_{m,k}}\left\{ \tau p^p_k \text{tr}\{\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k}\} + {\bar K}_{m,k}a_{m,k}||\mathbf{\bar{h} }_{m,k}||^2\right\} \\
\end{split}
\end{equation}

 Here, we note that \(\mathbf{\hat h}_{m,k}\) and \(\mathbf{\hat h}_{m,k'}\) are correlated if \(\{k,k'\} \in \mathcal{P}_k\). Therefore, we separately derive the interference's expression. First, if the \(k'\)-th user does not share the same pilot with the user \(k\), i.e., \(\{k,k'\} \notin \mathcal{P}_k\), then \(\mathbf{\hat h}_{m,k}\) and \(\mathbf{h}_{m,k'}\) are independent and we have
 \begin{equation}
\label{MRC_UIkk1}
\begin{split}
 &\mathbb{E} \left( {{{\left| {{\rm{U}}{{\rm{I}}_{k,k'}}} \right|}^2}} \right)\\
 =  &\mathbb{E} \left\{ {{{\left| {\sum\limits_{m \in {\mathcal{M}}_k} {w_{m,k}\sqrt {p_{k'}^d} {{\left( {{{{\bf{\hat h}}}_{m,k}}} \right)}^H}{{\bf{h}}_{m,k'}}} } \right|}^2}} \right\} \\
  =& {p_{k'}^d}\Big( \sum\limits_{m \in \mathcal{M}_k} w_{m,k}\sqrt{\bar K_{m,k}a_{m,k}\bar K_{m,k'}a_{m,k'}}\mathbf{\bar h}^H_{m,k}\mathbf{\bar{h} }_{m,k'} + w_{m,k}\sqrt{{\bar K}_{m,k'}a_{m,k'}}\mathbf{\widetilde q}^H_{m,k} \mathbf{\bar h}_{m,k'}\\
  + &w_{m,k}\sqrt{{\bar K}_{m,k}a_{m,k} a_{m,k'}} \mathbf{\bar h}^H_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'} +w_{m,k}\sqrt{a_{m,k'}}\mathbf{\widetilde q}^H_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'}\Big)^2\\
   =&  p^d_{k'} \left|\sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}\sqrt{\bar K_{m,k}\bar K_{m,k'}a_{m,k}a_{m,k'}}\mathbf{\bar h}^H_{m,k}\mathbf{\bar h}^H_{m,k'}\right|^2 \\
   +& p^d_{k'} \mathbb{E}\left\{ \left| \sum\limits_{m \in \mathcal{M}_k} w_{m,k}\sqrt{\bar K_{m,k'}a_{m,k'}}\mathbf{\widetilde q}^H_{m,k}\mathbf{\bar h}_{m,k'}\right|^2\right\} \\
  + &  p^d_{k'} \mathbb{E}\left\{ \left|\sum\limits_{m \in {\mathcal{M}}_k}  w_{m,k}\sqrt{{\bar K}_{m,k}a_{m,k} a_{m,k'}} \mathbf{\bar h}^H_{m,k}\boldsymbol{\Delta}_{m,k'} \mathbf{\widetilde h}_{m,k'} \right|^2\right\}\\ + & p^d_{k'} \mathbb{E}\left\{ \left| \sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}\sqrt{a_{m,k'}}\mathbf{\widetilde q}^H_{m,k} \boldsymbol{\Delta}_{m,k'}^{\frac{1}{2}}\mathbf{\widetilde h}_{m,k'} \right|^2\right\}
 \end{split}
 \end{equation}

\begin{equation}
    \begin{split}
        \mathbb{E}\left\{ \left| \sum\limits_{m \in \mathcal{M}_k} w_{m,k}\sqrt{\bar K_{m,k'}a_{m,k'}}\mathbf{\widetilde q}_{m,k}\mathbf{\bar h}_{m,k'}\right|^2\right\} &= \sum\limits_{m \in \mathcal{M}_k}w^2_{m,k} \bar K_{m,k'}a_{m,k'}\mathbb{E}\{\mathbf{\widetilde q}^H_{m,k}\mathbf{\bar h}_{m,k'}\mathbf{\bar h}^H_{m,k'} \mathbf{\widetilde q}_{m,k}\} \\
        & = \sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}\bar K_{m,k'}\tau p^p_k a_{m,k'} \mathbf{\bar h}^H_{m,k'} \mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k} \mathbf{R}_{m,k}\mathbf{h}_{m,k'}.
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
        &\mathbb{E}\left\{ \left|\sum\limits_{m \in {\mathcal{M}}_k}  w_{m,k}\sqrt{{\bar K}_{m,k}a_{m,k} a_{m,k'}} \mathbf{\bar h}^H_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'} \right|^2\right\}\\
        = &\sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}\bar K_{m,k}a_{m,k}a_{m,k'}\mathbb{E}\{\mathbf{\bar h}^H_{m,k}\boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{m,k'}\boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}  \mathbf{\bar h}_{m,k}\} \\
        = &\sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}\bar K_{m,k}a_{m,k}a_{m,k'}\mathbf{\bar h}^H_{m,k}\boldsymbol{\Delta}_{m,k'} \mathbf{\bar h}_{m,k}.
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
        \mathbb{E}\left\{ \left| \sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}\sqrt{a_{m,k'}}\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k'}^{\frac{1}{2}} \mathbf{\widetilde h}_{m,k'} \right|^2\right\} &= \sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}a_{m,k'}\mathbb{E}\{\mathbf{\widetilde q}^H_{m,k} \boldsymbol{\Delta}_{m,k'}^{\frac{1}{2}}\mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{m,k'}\boldsymbol{\Delta}_{m,k'}^{\frac{1}{2}}\mathbf{\widetilde q}_{m,k} \} \\
        & = \sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}\tau p^p_k a_{m,k'}\text{tr}\{\boldsymbol{\Delta}_{m,k'}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k} \mathbf{R}_{m,k}\}.
    \end{split}
\end{equation}


 If  the \(k'\)-th user share the same pilot with the user \(k\), i.e., \(\{k,k'\} \in \mathcal{P}_k\), then \(\mathbf{\hat h}_{m,k}\) and \(\mathbf{h}_{m,k'}\) are correlated, and we have
\begin{equation}
\label{MRC_UIkk2}
\begin{split}
 &\mathbb{E} \left( {{{\left| {{\rm{U}}{{\rm{I}}_{k,k'}}} \right|}^2}} \right)\\
 =  &\mathbb{E} \left\{ {{{\left| {\sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}{\sqrt {p_{k'}^d} {{\left( {{{{\bf{\hat h}}}_{m,k}}} \right)}^H}{{\bf{h}}_{m,k'}}} } \right|}^2}} \right\} \\
   =& {p_{k'}^d}\Big( \sum\limits_{m \in \mathcal{M}_k} w_{m,k}\sqrt{\bar K_{m,k}a_{m,k}\bar K_{m,k'}a_{m,k'}}\mathbf{\bar h}^H_{m,k}\mathbf{\bar{h} }_{m,k'} + w_{m,k}\sqrt{{\bar K}_{m,k'}a_{m,k'}}\mathbf{\widetilde q}^H_{m,k} \mathbf{\bar h}_{m,k'}\\
  + &w_{m,k}\sqrt{{\bar K}_{m,k}a_{m,k} a_{m,k'}} \mathbf{\bar h}^H_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'} +w_{m,k}\sqrt{a_{m,k'}}\mathbf{\widetilde q}^H_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'}\Big)^2\\
   =&  p^d_{k'} \left|\sum\limits_{m \in {\mathcal{M}}_k}w_{m,k} \sqrt{\bar K_{m,k}\bar K_{m,k'}a_{m,k}a_{m,k'}}\mathbf{\bar h}^H_{m,k}\mathbf{\bar h}^H_{m,k'}\right|^2 + p^d_{k'} \mathbb{E}\left\{ \left| \sum\limits_{m \in \mathcal{M}_k} w_{m,k}\sqrt{\bar K_{m,k'}a_{m,k'}}\mathbf{\widetilde q}^H_{m,k}\mathbf{\bar h}_{m,k'}\right|^2\right\} \\
  + &  p^d_{k'} \mathbb{E}\left\{ \left|\sum\limits_{m \in {\mathcal{M}}_k}  w_{m,k}\sqrt{{\bar K}_{m,k}a_{m,k} a_{m,k'}} \mathbf{\bar h}^H_{m,k}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'} \right|^2\right\} +p^d_{k'} \mathbb{E}\left\{ \left| \sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}\sqrt{a_{m,k'}}\mathbf{\widetilde q}^H_{m,k}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'} \right|^2\right\}\\
  +& 2 p^d_{k'} \text{Re}\left\{ \sum\limits_{m \in \mathcal{M}_k}\sum\limits_{n \in \mathcal{M}_k} w_{m,k}w_{n,k}\sqrt{\bar K_{m,k}a_{m,k}\bar K_{m,k'}a_{m,k'} a_{n,k'}}\mathbb{E}\{\mathbf{\bar h}^H_{m,k}\mathbf{\bar{h} }_{m,k'} \mathbf{\widetilde h}^H_{n,k'} \boldsymbol{\Delta}^{\frac{1}{2}}_{n,k'}\mathbf{\widetilde q}_{n,k}\} \right\}.
 \end{split}
 \end{equation}
In the following, we calculate the terms in (\ref{MRC_UIkk2}). The second and third terms are derived, and thus we derive the term \( \mathbb{E}\left\{ \left| \sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}\sqrt{a_{m,k'}}\mathbf{\widetilde q}^H_{m,k}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'} \right|^2\right\}\), which is given by
\begin{equation}
\label{UIKK2c}
    \begin{split}
    &\mathbb{E}\left\{ \left| \sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}\sqrt{a_{m,k'}}\mathbf{\widetilde q}^H_{m,k}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'} \right|^2\right\}\\
    =& \sum\limits_{m \in {\mathcal{M}}_k}\sum\limits_{n \in {\mathcal{M}}_k} w_{m,k}w_{n,k}\sqrt{a_{m,k'}a_{n,k'}}\mathbb{E}\{\mathbf{\widetilde q}^H_{m,k}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{n,k'}  \boldsymbol{\Delta}^{\frac{1}{2}}_{n,k'}\mathbf{\widetilde q}_{n,k}\} \\
    =& \sum\limits_{m \in {\mathcal{M}}_k}\sum\limits_{n \neq m} w_{m,k}w_{n,k}\sqrt{a_{m,k'}a_{n,k'}}\mathbb{E}\{\mathbf{\widetilde q}^H_{m,k}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{n,k'} \boldsymbol{\Delta}^{\frac{1}{2}}_{n,k'} \mathbf{\widetilde q}_{n,k} \}\\
    &+  \sum\limits_{m \in {\mathcal{M}}_k} w^2_{m,k}a_{m,k'} \mathbb{E}\{\mathbf{\widetilde q}^H_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{m,k'}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde q}_{m,k}\}\\ 
    \end{split}
\end{equation}

The first term in (\ref{UIKK2c}) is given by 
\begin{equation}
    \begin{split}
       & \mathbb{E}\{\mathbf{\widetilde q}^H_{m,k}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{n,k'} \boldsymbol{\Delta}^{\frac{1}{2}}_{n,k'} \mathbf{\widetilde q}_{n,k} \} \\
        =& \tau^2 p^p_k p^p_{k'}\sqrt{a_{m,k'}a_{n,k'}} \text{tr}\{ \boldsymbol{\Delta}_{m,k'} \mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k} \}  \text{tr}\{ \boldsymbol{\Delta}_{n,k'} \mathbf{R}_{n,k}\boldsymbol{\Psi}_{n,k} \} .
    \end{split}
\end{equation}

The second term in (\ref{UIKK2c}) can be calculated as
\begin{equation}
    \begin{split}
    & \mathbb{E}\{\mathbf{\widetilde q}^H_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{m,k'}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde q}_{m,k}\}\\
         = &\left| \Big( \sqrt{\tau p_k^p}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\sum_{j \in \mathcal{P}_k}\sqrt{\tau p^p_j a_{m,j}}\boldsymbol{\Delta}^{\frac{1}{2}}_{m,j}\mathbf{\widetilde h}_{m,j} +{\bf{n}}_{m,k}^p \Big)^H \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'}\right|^2 \\
    %= & \tau p_k^p \left| \Big(\sum_{j \in \mathcal{P}_k}\sqrt{\tau p^p_j a_{m,j}}\mathbf{\widetilde h}_{m,j} +{\bf{n}}_{m,k}^p \Big)^H \mathbf{\widetilde h}^H_{m,k'}\right|^2 \\
    =&  \tau p_k^p \mathbb{E}\left\{\sum_{j \in \mathcal{P}_k} \tau p^p_ja_{m,j} \mathbf{\widetilde h}^H_{m,j}\boldsymbol{\Delta}^{\frac{1}{2}}_{m,j} \boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{m,k'}\boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\boldsymbol{\Delta}^{\frac{1}{2}}_{m,j}\mathbf{\widetilde h}_{m,j} \right\} \\
    &+ \tau p_k^p |{(\bf{n}}_{m,k}^p)^H\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{ \widetilde h}_{m,k'}|^2 \\
    = & \tau p_k^p \sigma^2 \text{tr}\{\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \boldsymbol{\Delta}_{m,k'}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\} \\
    +& \tau p_k^p \sum\limits_{j \in \mathcal{P}_k}\tau p^p_j a_{m,j}\text{tr}\{ \boldsymbol{\Delta}_{m,j}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \boldsymbol{\Delta}_{m,k'}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\} \\
    +& \tau^2 p_k^p p_{k'}^pa_{m,k'}\text{tr}\{\boldsymbol{\Delta}_{m,k'}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \}\text{tr}\{\boldsymbol{\Delta}_{m,k'}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \} \\
    = &\tau^2 p_k^p p_{k'}^pa_{m,k'} \text{tr}\{\boldsymbol{\Delta}_{m,k'}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \}\text{tr}\{\boldsymbol{\Delta}_{m,k'}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \} + \tau p_k^p \text{tr}\{\mathbf{R}_{m,k} \boldsymbol{\Delta}_{m,k'}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\} .   
    \end{split}
\end{equation}

\(\mathbb{E}\{\mathbf{\bar h}^H_{m,k}\mathbf{\bar{h} }_{m,k'} \mathbf{\widetilde h}^H_{n,k'} \boldsymbol{\Delta}^{\frac{1}{2}}_{n,k'}\mathbf{\widetilde q}_{n,k}\}\) can be calculated as
\begin{equation}
    \begin{split}
        \mathbb{E}\{\mathbf{\bar h}^H_{m,k}\mathbf{\bar{h} }_{m,k'} \mathbf{\widetilde h}^H_{n,k'} \boldsymbol{\Delta}^{\frac{1}{2}}_{n,k'}\mathbf{\widetilde q}_{n,k}\} =  \tau\sqrt{ p^p_{k'}p^p_{k}a_{n,k'}} \mathbf{\bar h}^H_{m,k}\mathbf{\bar{h} }_{m,k'} \text{tr}\{\boldsymbol{\Delta}_{n,k'}\mathbf{R}_{n,k}\boldsymbol{\Psi}_{n,k}\}.
    \end{split}
\end{equation}



The term $\mathbb{E}\left( \left| {{\rm{LS}}_{k}} \right|^2 \right)$ is given by
\begin{equation}
\setlength\abovedisplayskip{5pt}
\setlength\belowdisplayskip{5pt}
\label{MRC_LSk}
\begin{split}
&\mathbb{E} \left\{ {{{\left| {{\rm{LS}}_{k}} \right|}^2}} \right\}  
= {p_k^d} \mathbb{E} \left\{ {{{\left| {\sum\limits_{m \in {\mathcal{M}}_k}{{{\left( {{\bf{\hat h}}_{m,k}} \right)}^H}{\bf{h}}_{m,k} } -  {{\rm{DS}}_{k}}} \right|}^2}} \right\}   \\
%=& p^d_k \mathbb{E}\{ |\sum\limits_{m \in \mathcal{M}_k}\mathbf{\widetilde h}^H_{m,k}\mathbf{\widetilde h}_{m,k}|^2\} + p^d_k \mathbb{E}\{ |\sum\limits_{m \in \mathcal{M}_k}\mathbf{\widetilde h}^H_{m,k}\mathbf{\widetilde e}_{m,k}|^2\} -{{\rm{DS}}^2_{k}}\\
= &{p_k^d}\Big(\sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}\sqrt{\bar K_{m,k}a_{m,k}}\mathbf{\widetilde q}^H_{m,k} \mathbf{\bar{h} }_{m,k} + w_{m,k}\sqrt{\bar K_{m,k}a_{m,k}a_{m,k}} \mathbf{\bar{h} }^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\\
 & +w_{m,k}\sqrt{a_{m,k}}\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k} - {w_{m,k}}\tau p^p_k \text{tr}\{\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k}\}\Big)^2 \\
 =& {p_k^d} \sum\limits_{m \in {\mathcal{M}}_k} w^2_{m,k}\bar K_{m,k}a_{m,k} \mathbb{E}\{|\mathbf{\widetilde q}^H_{m,k}\mathbf{\bar{h} }_{m,k} |^2\} + {p_k^d} \sum\limits_{m \in {\mathcal{M}}_k}  w^2_{m,k}\bar K_{m,k}a_{m,k}a_{m,k} \mathbb{E}\{|\mathbf{\bar{h} }^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k} |^2\}\\
  &+  {p_k^d} \mathbb{E}\left\{ \sum\limits_{m \in {\mathcal{M}}_k}\sum\limits_{n \in {\mathcal{M}}_k} w_{m,k}w_{n,k}\sqrt{a_{m,k} a_{n,k}}\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\mathbf{\widetilde{h} }^H_{n,k}\boldsymbol{\Delta}_{n,k}^{\frac{1}{2}}\mathbf{\widetilde q}_{n,k}\right\}\\
  &+ {p_k^d}\Big(\sum\limits_{m \in {\mathcal{M}}_k}{w_{m,k}}\tau p^p_k \text{tr}\{\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k}\}\Big)^2 \\
  & - 2{p_k^d}\text{Re}\left\{\sum\limits_{m \in {\mathcal{M}}_k}\sum\limits_{n \in {\mathcal{M}}_k}  \tau p^p_k \text{tr}\{\mathbf{R}_{n,k}\boldsymbol{\Psi}_{n,k}\mathbf{R}_{n,k}\}w_{m,k}w_{n,k}\sqrt{a_{m,k}}\mathbb{E}\{\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\}\right\} .
 \end{split}
\end{equation}

Then, the first term \(\mathbb{E}\{|\mathbf{\widetilde q}^H_{m,k}\mathbf{\bar{h} }_{m,k} |^2\}\) of (\ref{MRC_LSk}) can be calculated as
\begin{equation}
    \begin{split}
        \mathbb{E}\{|\mathbf{\widetilde q}^H_{m,k}\mathbf{\bar{h} }_{m,k} |^2\} = \tau p^p_k \mathbf{\bar h}^H_{m,k} \mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k}\mathbf{\bar h}_{m,k}.
    \end{split}
\end{equation}
The second term \(\mathbb{E}\{|\mathbf{\bar{h} }^H_{m,k}\mathbf{\widetilde{h} }_{m,k} |^2\}\) is given by
\begin{equation}
    \mathbb{E}\{|\mathbf{\bar{h} }^H_{m,k}\mathbf{\widetilde{h} }_{m,k} |^2\} = \mathbf{\bar h}^H_{m,k}\boldsymbol{\Delta}_{m,k}\mathbf{\bar h}_{m,k}.
\end{equation}
The third term in (\ref{MRC_LSk}) can be written as
\begin{equation}
\begin{split}
    &\mathbb{E}\left\{ \sum\limits_{m \in {\mathcal{M}}_k}\sum\limits_{n \in {\mathcal{M}}_k} w_{m,k}w_{n,k}\sqrt{a_{m,k} a_{n,k}}\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\mathbf{\widetilde{h} }^H_{n,k}\boldsymbol{\Delta}_{n,k}^{\frac{1}{2}}\mathbf{\widetilde q}_{n,k}\right\}  \\
    =& \mathbb{E}\left\{ \sum\limits_{m \in {\mathcal{M}}_k}\sum\limits_{n \neq m}w_{m,k}w_{n,k}\sqrt{a_{m,k} a_{n,k}}\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\mathbf{\widetilde{h} }^H_{n,k}\boldsymbol{\Delta}_{n,k}^{\frac{1}{2}}\mathbf{\widetilde q}_{n,k}\right\} \\
    +& \mathbb{E}\left\{ \sum\limits_{m \in {\mathcal{M}}_k} w^2_{m,k}a_{m,k}\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\mathbf{\widetilde{h} }^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde q}_{m,k}\right\} \\
    %=& \sum\limits_{m \in {\mathcal{M}}_k}\sum\limits_{n \neq m}(N\tau p^p_k a_{m,k}a_{n,k})^2b_{m,k}b_{n,k}  \\
    %+&  \sum\limits_{m \in {\mathcal{M}}_k}a_{m,k}\tau p^p_k a^2_{m,k}b^2_{m,k}\Big(\sum\limits_{j \in \mathcal{P}_k}\sqrt{\tau p^p_{m,j}a_{m,j}}\mathbf{\widetilde h}^H_{m,j}\mathbf{\widetilde h}_{m,k}+(\mathbf{n}^p_{m,k})^H\mathbf{\widetilde h}_{m,k}\Big)\\
    %\times & \Big(\sum\limits_{j \in \mathcal{P}_k}\sqrt{\tau p^p_{m,j}a_{m,j}}\mathbf{\widetilde h}^H_{m,j}\mathbf{\widetilde h}_{m,k}+(\mathbf{n}^p_{m,k})^H\mathbf{\widetilde h}_{m,k}\Big)^H\\
    =&  \Big(\tau p^p_k \sum \limits_{m \in \mathcal{M}_k}w_{m,k} a_{m,k}\text{tr}\{\boldsymbol{\Delta}_{m,k}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}   \} \Big)^2 + \sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}\tau p_k^p a_{m,k}\text{tr}\{\mathbf{R}_{m,k} \boldsymbol{\Delta}_{m,k}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\}. 
\end{split} 
\end{equation}
The fourth term \(\mathbb{E}\{\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\}\) is calculated as
\begin{equation}
   \mathbb{E}\{\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\} = \tau p^p_k \sqrt{a_{m,k}} \text{tr}\{\boldsymbol{\Delta}_{m,k}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\}.
\end{equation}
By substituting all terms into (\ref{MRC_LSk}), we have
\begin{equation}
    \begin{split}
        \mathbb{E} \left\{ {{{\left| {{\rm{LS}}_{k}} \right|}^2}} \right\}  & =   {p_k^d} \sum\limits_{m \in \mathcal{M}_k}w^2_{m,k} \bar K_{m,k}\tau p^p_k a_{m,k} \mathbf{\bar h}^H_{m,k} \mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k} \mathbf{R}_{m,k}\mathbf{h}_{m,k}\\
        & + p_k^d \sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}\bar K_{m,k}a_{m,k}a_{m,k}\mathbf{\bar h}^H_{m,k}\boldsymbol{\Delta}_{m,k} \mathbf{\bar h}_{m,k}\\
        &+ p_k^d \sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}\tau p_k^p a_{m,k}\text{tr}\{\mathbf{R}_{m,k} \boldsymbol{\Delta}_{m,k}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\}
       % &+ {p_k^d} \sum\limits_{m \in {\mathcal{M}}_k} a_{m,k} N\tau p_k^pa^2_{m,k}b_{m,k}(Nb_{m,k}\tau p^p_{k}a_{m,k}+1) \\
        %& - 2{p_k^d}\text{Re}\left\{\sum\limits_{m \in {\mathcal{M}}_k}  N \tau p^p_k a^{5/2}_{m,k}b_{m,k}N \tau p^p_{k}a^{3/2}_{m,k}b_{m,k}\right\}-
    \end{split}
\end{equation}
 %( N \tau p^p_k a^2_{m,k}b_{m,k})^2

Finally, we compute $\mathbb{E}\left( \left| {{\rm{N}}_{k}} \right|^2 \right)$, which is given by
\begin{equation}
\label{MRC_Nk}
\begin{split}
    \mathbb{E} \left( {{{\left| {{{\rm{N}}_k}} \right|}^2}} \right) &= \mathbb{E}\{|\sum\limits_{m \in \mathcal{M}_k} \sqrt{w_{m,k}} {{{\left( {{\bf{ \hat h}}_{m,k}} \right)}^H}{\bf{n}}_m}|^2\} \\
        & = \sum\limits_{m \in \mathcal{M}_k}{w^2_{m,k}}\Big( \tau p^p_k  \text{tr}\{\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k}\} + \bar K_{m,k}a_{m,k} \mathbf{\bar h}^H_{m,k}\mathbf{\bar h}_{m,k}\Big)\sigma^2 .
\end{split}
\end{equation}

Substituting all these results into (\ref{kth_SINR}), we obtain \(1 \) in (\ref{MRC_SINR_LB}).
\end{appendices}
